Understanding and Mitigating Overfitting in Prompt Tuning for Vision-Language Models

Pretrained vision-language models (VLMs) such as CLIP have shown impressive generalization capability in downstream vision tasks with appropriate text prompts. Instead of designing prompts manually, Context Optimization (CoOp) has been recently proposed to learn continuous prompts using taskspecific training data. Despite the performance improvements on downstream tasks, several studies have reported that CoOp suffers from the overfitting issue in two aspects: (i) the test accuracy on base classes first improves and then worsens during training;(ii) the test accuracy on novel classes keeps decreasing. However, none of the existing studies can understand and mitigate such overfitting problems. In this study, we first explore the cause of overfitting by analyzing the gradient flow. Comparative experiments reveal that CoOp favors generalizable and spurious features in the early and later training stages, respectively, leading to the non-overfitting and overfitting phenomena. Given those observations, we propose Subspace Prompt Tuning (SubPT) to project the gradients in back-propagation onto the low-rank subspace spanned by the early-stage gradient flow eigenvectors during the entire training process and successfully eliminate the overfitting problem. In addition, we equip CoOp with a Novel Feature Learner (NFL) to enhance the generalization ability of the learned prompts onto novel categories beyond the training set, needless of image training data. Extensive experiments on 11 classification datasets demonstrate that SubPT+NFL consistently boost the performance of CoOp and outperform the state-of-the-art CoCoOp approach. Experiments on more challenging vision downstream tasks, including open-vocabulary object detection and zero-shot semantic segmentation, also verify the effectiveness of the proposed method. Codes can be found at https://tinyurl.com/mpe64f89.

==> Figures/base-and-novel-bak.tex <==
\begin{figure*}[t]
\centering
\scalebox{0.98}{
\subfloat[\footnotesize Base class test set accuracy]{
\includegraphics[width=0.24\linewidth]{Images/BaseAccuracy-crop.pdf}
\label{fig: base accuracy}
}
\hfill
\hfill
\subfloat[\footnotesize Novel class test set accuracy]{
\includegraphics[width=0.24\linewidth]{Images/NovelAccuracy-crop.pdf}
\label{fig: novel accuracy}
}
\hfill
\hfill
\subfloat[\footnotesize Train set accuracy]{
\includegraphics[width=0.24\linewidth]{Images/TrainAccuracy-crop.pdf}
\label{fig: train accuracy}
}
\hfill
\hfill
\subfloat[\footnotesize Train set loss]{
\includegraphics[width=0.24\linewidth]{Images/TrainLoss-crop.pdf}
\label{fig: train loss}
}
}
\vspace{1mm}
\caption{\textbf{Illustrations on two aspects of overfitting problem in CoOp and CoCoOp}. The dataset is Caltech101. (a) The base class test set accuracy first gets better than gets worse during the training processes of CoOp and CoCoOp. (b) The novel class test set accuracy keeps decreasing and is far below that of zero-shot CLIP. (c) and (d) show that there is no clue of overfitting when monitoring the training process.}
\label{fig: base and novel}
\end{figure*}

==> Tables/base2novel-bak.tex <==
\begin{table*}[t]
\centering
%\scriptsize
\renewcommand\arraystretch{1.15}
\caption{Comparison with state-of-the-art approaches on base-to-novel generalization. HM stands for Harmonic Mean. \textbf{Best} and \textbf{\underline{second best}} results are highlighted.}
\vspace{-1.mm}
\scalebox{1.05}{
\begin{tabular}{l | c c c | c c c | c c c}
\hline
       & \multicolumn{3}{c|}{\textbf{Average}} & \multicolumn{3}{c|}{ImageNet} & \multicolumn{3}{c}{Caltech101} \\
       & Base  & Novel & HM    & Base  & Novel & HM    & Base  & Novel & HM    \\\hline
Zero-shot CLIP   & 65.17 & \textbf{69.05} & 66.94 & 64.39 & 60.05 & 62.14 & 90.77 & \textbf{\underline{91.05}} & 90.91 \\
CoOp   & 72.10 & 58.75 & 63.90 & 64.25 & 54.99 & 59.26 & 94.00 & 87.37 & 90.56 \\
CoCoOp & 71.91 & 60.42 & 65.19 & \textbf{\underline{66.49}} & 58.54 & 62.26 & 94.36 & 86.10 & 90.04 \\
\rowcolor{black!10} CoOp + \textit{Sub}PT
       & \textbf{\underline{72.57}} & 62.30 & 66.37 & \textbf{66.91} & \textbf{\underline{60.32}} & 63.44 & 94.35 & 89.27 & 91.74 \\
\rowcolor{black!10} CoOp + \textit{Sub}PT + NFL$_{unknown}$
       & 72.74 & 65.04 & \textbf{\underline{68.17}} & 66.32 & 60.22 & 63.12 & \textbf{94.86} & 90.72 & \textbf{\underline{92.74}} \\
\rowcolor{black!10} CoOp + \textit{Sub}PT + NFL$_{known}$   
       & \textbf{72.96} & \textbf{\underline{66.91}} & \textbf{69.32} & 66.14 & \textbf{61.16} & \textbf{63.55} & \textbf{\underline{94.77}} & \textbf{92.10} & \textbf{93.42} \\\hline
       & \multicolumn{3}{c|}{Oxford Pets} & \multicolumn{3}{c|}{Stanford Cars} & \multicolumn{3}{c}{Flowers 102} \\
       & Base  & Novel & HM    & Base  & Novel & HM    & Base  & Novel & HM    \\\hline
Zero-shot CLIP   & 90.06 & 94.18 & 92.07 & 55.32 & \textbf{66.65} & 60.46 & 69.14 & \textbf{73.97} & 71.47 \\
CoOp   & 89.67 & 92.34 & 90.99 & 62.57 & 55.24 & 58.68 & 86.80 & 63.55 & 73.38 \\
CoCoOp & 87.75 & 90.16 & 88.94 & 61.32 & 56.97 & 59.07 & 87.08 & 62.62 & 72.85 \\
\rowcolor{black!10} CoOp + \textit{Sub}PT
       & 90.96 & 92.60 & 91.77 & \textbf{62.67} & 58.83 & 60.69 & \textbf{88.75} & 63.22 & 73.84 \\
\rowcolor{black!10} CoOp + \textit{Sub}PT + NFL$_{unknown}$
       & \textbf{\underline{91.62}} & \textbf{95.41} & \textbf{93.48} & \textbf{\underline{62.62}} & 62.32 & \textbf{\underline{62.47}} & 87.09 & 64.40 & \textbf{\underline{74.05}} \\
\rowcolor{black!10} CoOp + \textit{Sub}PT + NFL$_{known}$   
       & \textbf{91.65} & \textbf{\underline{95.32}} & 93.45 & 61.08 & \textbf{\underline{65.82}} & \textbf{63.36} & \textbf{\underline{88.19}} & \textbf{\underline{71.68}} & \textbf{79.08} \\\hline
       & \multicolumn{3}{c|}{Food 101} & \multicolumn{3}{c|}{FGVC Aircraft} & \multicolumn{3}{c}{SUN 397} \\
       & Base  & Novel & HM    & Base  & Novel & HM    & Base  & Novel & HM    \\\hline
Zero-shot CLIP   & \textbf{83.59} & \textbf{85.01} & \textbf{84.29} & 18.79 & \textbf{25.97} & \textbf{\underline{21.80}} & 66.78 & 70.51 & 68.59 \\
CoOp   & 78.59 & 77.86 & 78.22 & \textbf{\underline{22.63}} & 16.92 & 19.36 & 71.16 & 62.20 & 66.38 \\
CoCoOp & 78.53 & 78.31 & 78.42 & 21.67 & 16.68 & 18.85 & 70.18 & 64.29 & 67.11 \\
\rowcolor{black!10} CoOp + \textit{Sub}PT 
       & 80.76 & 80.85 & 80.80 & 19.09 & 21.78 & 20.35 & 72.37 & 68.14 & 70.19 \\
\rowcolor{black!10} CoOp + \textit{Sub}PT + NFL$_{unknown}$
       & \textbf{\underline{82.61}} & 83.94 & \textbf{\underline{83.27}} & 18.85 & 23.94 & 21.09 & \textbf{\underline{72.68}} & \textbf{\underline{70.56}} & \textbf{\underline{71.60}} \\
\rowcolor{black!10} CoOp + \textit{Sub}PT + NFL$_{known}$   
       & 82.20 & \textbf{\underline{84.14}} & 83.16 & \textbf{22.99} & \textbf{\underline{25.13}} & \textbf{24.01} & \textbf{73.35} & \textbf{71.44} & \textbf{72.38} \\\hline
       & \multicolumn{3}{c|}{DTD} & \multicolumn{3}{c|}{EuroSAT} & \multicolumn{3}{c}{UCF 101} \\
       & Base  & Novel & HM    & Base  & Novel & HM    & Base  & Novel & HM    \\\hline
Zero-shot CLIP   & 54.17 & \textbf{56.16} & 55.15 & 54.83 & \textbf{66.18} & 59.97 & 69.03 & \textbf{69.82} & \textbf{\underline{69.42}} \\
CoOp   & 66.09 & 42.75 & 51.92 & 85.10 & 35.67 & 50.27 & 72.23 & 57.33 & 63.92 \\
CoCoOp & 65.74 & 41.55 & 50.92 & \textbf{85.74} & \textbf{\underline{51.97}} & \textbf{64.71} & 72.13 & 57.44 & 63.95 \\
\rowcolor{black!10} CoOp + \textit{Sub}PT
       & \textbf{\underline{66.28}} & 46.50 & 54.66 & 81.98 & 40.79 & 54.48 & \textbf{74.10} & 63.01 & 68.11 \\
\rowcolor{black!10} CoOp + \textit{Sub}PT + NFL$_{unknown}$
       & \textbf{66.36} & 47.67 & \textbf{\underline{55.48}} & 83.42 & 50.97 & \textbf{\underline{63.28}} & \textbf{\underline{73.73}} & 65.28 & 69.25 \\
\rowcolor{black!10} CoOp + \textit{Sub}PT + NFL$_{known}$   
       & 63.73 & \textbf{\underline{52.33}} & \textbf{57.47} & \textbf{\underline{85.71}} & 49.26 & 62.56 & 72.71 & \textbf{\underline{67.59}} & \textbf{70.06}
\\\hline
\end{tabular}
}
\label{tab: base2novel}
\end{table*}

==> Tables/prompt_template.tex <==
\begin{table}[t]
\centering
%\scriptsize
\renewcommand\arraystretch{1.15}
\caption{Prompt template for computing zero-shot CLIP text features.}
\vspace{-1.mm}
\scalebox{0.98}{
\begin{tabular}{c c}
\hline
id & Prompt template \\\hline
1  & itap of a [CLASS]. \\
2  & a bad photo of the [CLASS]. \\
3  & a origami [CLASS]. \\
4  & itap of a [CLASS]. \\
5  & itap of a [CLASS]. \\
6  & itap of a [CLASS]. \\
7  & itap of a [CLASS]. 
\\\hline
\end{tabular}
}
\label{tab: template}
\end{table}
